Active Open-Vocabulary Recognition: Let Intelligent Moving Mitigate CLIP Limitations

Active recognition, which allows intelligent agents to explore observations for better recognition performance, serves as a prerequisite for various embodied AI tasks, such as grasping, navigation and room arrangements. Given the evolving environment and the multitude of object classes, it is impractical to include all possible classes during the training stage. In this paper, we aim at advancing active open-vocabulary recognition, empowering embodied agents to actively perceive and classify arbitrary objects. However, directly adopting recent open-vocabulary classification models, like Contrastive Language Image Pretraining (CLIP), poses its unique challenges. Specifically, we observe that CLIP's performance is heavily affected by the viewpoint and occlusions, compromising its reliability in unconstrained embodied perception scenarios. Further, the sequential nature of observations in agent-environment interactions necessitates an effective method for integrating features that maintains discriminative strength for open-vocabulary classification. To address these issues, we introduce a novel agent for active open-vocabulary recognition. The proposed method leverages inter-frame and inter-concept similarities to navigate agent movements and to fuse features, without relying on class-specific knowledge. Compared to baseline CLIP model with 29.6% accuracy on ShapeNet dataset, the proposed agent could achieve 53.3% accuracy for open-vocabulary recognition, without any fine-tuning to the equipped CLIP model. Additional experiments conducted with the Habitat simulator further affirm the efficacy of our method.

==> sec/0_abstract.tex <==
\begin{abstract}
% Pretrained open-vocabulary image classification model
% Contrastive language image pretraining (CLIP)

% 0. Active recognition, which is XXX, is the basic requirements for different embodied AI tasks, like grasping, navigation and room arrangements.
% 1. The ability to recognize open-vocabulary classes is crutial to embodied agents as the environments to explore is inherently unseen and evolving. 
% 1.5 When embeding pretrained vision recognition modules to robots, several different challenges emerge.
%  a. View
%  b. Occlusion
%  c. Distance
% 2. CLIP models have significant power for many downstream tasks, especially when related to open-vocabulary capabilities. Their ability to claissify objects by arbitray text inputs aligns with our expetation for embodied agents.
% 3. However, after investigating recent CLIP visual backbones, we find the CLIP model is very sensitive to the viewpoint, making the recognition fails at randomly chosen viewpoints, which also consolidate the incentive for the agent the choose discrimitive views for the CLIP model.
% 4. Compared to vanilla CLIP model with 29.2 mAP on ShapeNet dataset, the proposed active recognition model could achieve a 41.1 mAP after taking 5 movements without changing the CLIP model.
% Other experiments on Habitat and AI2THOR indoor simulators also validate the proposed method on achieving superior open-vocabulary recognition performance compared to CLIP model.

Active recognition, which allows intelligent agents to explore observations for better recognition performance, serves as a prerequisite for various embodied AI tasks, such as grasping, navigation and room arrangements.
Given the evolving environment and the multitude of object classes, it is impractical to include all possible classes during the training phase.
In this paper, we aim at advancing active open-vocabulary recognition, empowering embodied agents to actively perceive and classify arbitrary objects.
However, directly adopting recent open-vocabulary classification models, like Contrastive Language Image Pretraining (CLIP), poses its unique challenges.
Specifically, we observe that CLIP's performance is heavily affected by the viewpoint and occlusions, compromising its reliability in unconstrained embodied perception scenarios. 
Further, the sequential nature of observations in agent-environment interactions necessitates an effective method for aggregating features that maintains discriminative strength for open-vocabulary classification.
To address these issues, we introduce a novel unified approach for active open-vocabulary recognition.
The proposed method leverages inter-frame and inter-concept similarities to navigate agent movements and to fuse features, without relying on class-specific knowledge.
Compared to baseline CLIP model with 29.2\% accuracy on ShapeNet dataset, the proposed active recognition agent could achieve 41.1\% accuracy in its final step, without any fine-tuning to the equipped CLIP model.
Additional experiments conducted with the Habitat and AI2-THOR simulators further affirm the efficacy of our method.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
% Main Story Logic:
% 1. Embodied AI requires active recognition. 
%       Active recognition is a must for most embodied AI tasks. Every task needs identify the target before further motion planning.
% 2. Object categories in household scenario is versatile. 
%       Covering all classes in a training dataset is impractical and requires extensive resources. -> Requires open-vocabulary recognition, What is OVR?
% 3. Recent pretrained vision language models, like CLIP, show their progress in open-vocabulary recognition. 
%       Like human, they align visual embedings to language concept to enable zero-shot like recognition during testing.
% 4. Directly applying CLIP has its own challenges. (Demonstrative Figures)
%       a. These methods are trained with image-language pairs collected from internet. Most of these training images are differentiable between classes and in a good viewpoint. However, they are passive recognition methods and are not designed for embodied recognition scenarios, where viewing conditions are highly unconstrained.
%       b. Sequential input. How to aggregate sequential knowledge for ov classes that are not seen during training. Also, the aggregated feature needs to be discriminative for ov classification.
% 5. How do we address these challenges.
%       a. Active recognition. Let agents find discriminative views. Model it as a RL problem. Also discard the input-semantic relations during policy learning to enable it for ov classification.
%       b. Interframe and interconcept similarity measure to give feature aggregation weights.
% 6. Advantages:
%       a. Over baseline CLIP model.
%       b. Over other heuristic policies.

% Pages 1 - 1.5
% ------ P1  ------
% Active recognition
% 1. The history of active recognition.
% 2. Why active recognition is important. The intuition behind active recognition, like human.
% 3. The application of active recognition.
% 4. Previous active recognition is constrained to a prefix set.
% 5. Why we need open-vocabulary for embodied agents?

% -----------------

% ------ P2  ------
% Open-vocabulary recognition
% 1. What is ovr? Task definition. Relationship with zero-shot.
% 2. What is the motivation for ovr? resources for annotating, more general application scenarios.
% 3. Current progress in ovr.
% 4. Why these ovr works.
% 5. What are the current applications for ovr? ov detection, etc

% -----------------

% ------ P3  ------
% Limit of CLIP
% 1. What is CLIP, how CLIP is trained, what can CLIP do? Even human can recognize abundant classes, we still need to change viewpoints instead of with one image.
% 2. What is the limitation of CLIP, why these limitations happen?
% 3. Statistics on ShapeNet and Habitat. Different CLIP models give the same limitation.
% 4. Embodied perception scenario is unconstrained. Give examples.
% 5. We need to accomodate CLIP on to the embodied agent.

% -----------------

% ------ P4  ------
% Challenges of adopting CLIP into active recognition.
% 1. Generalization ability of policy.
% 2. Previous AR are all closed set. Their policy is highly related to the class. Making these method not directly appliable.
% 3. Feature aggregation challenge. Previous AR aggregate features with one trainable encoder.
% 4. Our method design. 
%   a. Purely attention based local feature integration. Why?
%   b. Disentangele between semantic-specific knowledge to policy. Why?

% -----------------

% ------ P5  ------
% Experiments and advantages.
% 1. On ShapeNet. Why do we choose ShapeNet, it is more clear, the result is directly related to the viewpoint.
% 2. On Habitat. Popular for embodied AI tasks.
% 3. Our advantages over baseline CLIP.
% 4. Our advantages over heuristic policies.

% -----------------

% ------ P6  ------
% Contributions
% 1. Study CLIP limitations in embodied perception scenarios
% 2. Propose active open-vocabulary task and a corresponding approach. One sentence about proposed approach.
% 3. Our advantange in experiments, show the need to do AOVR for embodied agents.

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figure/replace.pdf}
    \caption{\todo{Needs two subfigures. 1. Show what is active ov recognition. 2. The limit of passive recognition. 3. The limit of CLIP.}}
    \label{fig:clip_limit}
\end{figure}

==> sec/2_related_work.tex <==
\section{Related Work}
\label{sec:related}

% Pages 3/4 - 1
% 1. Embodied AI tasks - active recognition
%   a. Embodied AI tasks need recognition. 
%   b. Active recognition's history, all based on closed-world setting. Their visual encoders.
%   c. Continual learning in embodied AI to handle envolving environment.
\noindent{\bf{Active recognition.}}

% 2. Pretrained vision language models
%   a. CLIP and CLIP-based models.
%   b. CLIP in embodied AI tasks.
%   c. Studies of CLIP limitations.
%   d. CLIP feature aggregation methods.
\noindent{\bf{Pretrained vision language model.}}


% 3. Summarization

==> sec/3_clip_limit.tex <==
\section{Limitations in CLIP}
\label{sec:limit}

% Page 3/2 - 2
% ------ P1  ------
% Leading paragraph
% 1. The real recognition scenario of embodied agents.
% 2. Major challenge of embodied perception, can include some references from first-person vision.
% 3. What are the limitations of CLIP models that have been studied?
% 4. What aspects do we want to check with CLIP models? Viewpoint and occlusions. All classes are used for the study. In a fully ov recognition setting.
% 5. What are the CLIP models we choose? Why do we choose these CLIP models?

% -----------------


% ------ P2  ------
\subsection{Datasets for investigation}
% ShapeNet datasets
% 1. How do we prepare the dataset? From CAD models to 12*12 views.
% 2. How do we define viewpoint? How do we define occlusions?
\noindent{\bf{ShapeNet dataset.}}

% Habitat dataset
% 1. Why do we further test CLIP on Habitat? More real, more close to embodied AI tasks.
% 2. How do we collect the dataset? How do we define viewpoint? Why not occlusions?
\noindent{\bf{Habitat dataset.}}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figure/replace.pdf}
    \caption{\todo{Show two examples of our datasets to test limitations.}}
    \label{fig:dataset_limit}
\end{figure}

% -----------------

% ----- P3  ------
% Experiments on Viewpoint
\subsection{CLIP sensitivity to viewpoints}
% 1. How do we design the experiments? 
% 2. Result analysis.

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figure/replace.pdf}
    \caption{\todo{Viewpoint changing result on ShapeNet and Habitat.}}
    \label{fig:limit_view}
\end{figure}

% -----------------

% ----- P4  ------
% Experiments on Occlusion
\subsection{Impact of occlusion on CLIP}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figure/replace.pdf}
    \caption{\todo{Occlusion effect of CLIP on ShapeNet}}
    \label{fig:limit_occ}
\end{figure}
% -----------------

==> sec/4_method.tex <==
\section{Method}
\label{sec:method}
% Page 1
% Overall paragraph to describe the major components of this part.

\subsection{Problem setup and notation}
% 1. Discuse base, novel and open classes. And which one to use during training and testing.
% 2. Discuss active recognition setting.
%   a. Observation space, action space, etc.
%   b. Number of steps.
%   c. The objective of an active recognition agent.
%   d. The key component of an active recognition agent.

\subsection{Attention-based CLIP feature integration}
% 1. Why do we need feature integration for active recognition?
% 2. What is the specific needs for integrating CLIP features. As their similarity are measured with cosine similarity, it allows us to calculate the fused feature with weighted sum.
% 3. The advantage:
%   a. Not related to classes. Could be extended to the testing phase
%   b. Flexible to number of inliers.
%   c. Not affecting the open-set discriminative power.
% 4. Architecture. Training strategy and loss. Masking.


\subsection{Active open-vocabulary recognition agent}
% 1. The two parts of agent. Their architectures
% 2. How do we model the policy part.
% 3. Reward during training. The reward for shapenet and habitat is different. Explain the reason
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figure/replace.pdf}
    \caption{\todo{Draw the architecture of proposed method.}}
    \label{fig:method}
\end{figure}

==> sec/5_experiment.tex <==
\section{Experiment}
\label{sec:experiment}
% Page 3

\subsection{Datasets and experimental setup}
% Notes: We choose the most common classes as base classes because it is a solid assumtion to train policy on these classes.
% 1. Datasets
% 2. How do we split classes into base, novel and open.

\subsection{Implementations}

\subsection{Result on ShapeNet}
% 1. Different splits

\subsection{Result for indoor simulators}
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figure/replace.pdf}
    \caption{\todo{Show the result example on habitat.}}
    \label{fig:result}
\end{figure}

\subsection{Ablation studies}
% 1. Feature fusion strategy (split 20)
% 2. Direct semantic feature or similarity
% 3. Different CLIP architecture
% 4. op-k ablation (not important)

\subsection{Adversarial disturbance}
% 1. Random occlusion (no training needed)

==> sec/6_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
